OpenMixup: Open Mixup Toolbox and Benchmark for Visual Representation Learning

Mixup augmentation has emerged as a widely used technique for improving the generalization ability of deep neural networks (DNNs). However, the lack of standardized implementations and benchmarks has impeded recent progress, resulting in poor reproducibility, unfair comparisons, and conflicting insights. In this paper, we introduce OpenMixup, the first mixup augmentation codebase, and benchmark for visual representation learning. Specifically, we train 18 representative mixup baselines from scratch and rigorously evaluate them across 11 image datasets of varying scales and granularity, ranging from fine-grained scenarios to complex non-iconic scenes. We also open-source our modular codebase, including a collection of popular vision backbones, optimization strategies, and analysis toolkits, which not only supports the benchmarking but enables broader mixup applications beyond classification, such as self-supervised learning and regression tasks. Through experiments and empirical analysis, we gain observations and insights on mixup performance-efficiency trade-offs, generalization, and optimization behaviors, and thereby identify preferred choices for different needs. To the best of our knowledge, OpenMixup has facilitated several recent studies. We believe this work can further advance reproducible mixup augmentation research and thereby lay a solid ground for future progress in the community. The source code and user documents are available at \url{https://github.com/Westlake-AI/openmixup}.

==> 7_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% neurips2024 DB track %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{app:implementation}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \answerYes{See Section \ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerTODO{}
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerTODO{}
    \answerNA{}
  \item Did you include complete proofs of all theoretical results?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerTODO{}
    % \answerYes{In the supplemental material.}
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    % \answerTODO{}
    \answerYes{}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    % \answerTODO{}
    \answerYes{}
\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    % \answerTODO{}
    \answerYes{}
  \item Did you mention the license of the assets?
    % \answerTODO{}
    \answerNo{The used code and data are open-source and under the MIT license for research usage.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    % \answerTODO{}
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    % \answerTODO{}
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    % \answerTODO{}
    \answerNA{The used data has undergone ethical review.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}

\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/app_cub_fgvc_place.tex <==
\begin{table}[htb]
    \centering
    % \vspace{-1.0em}
    \caption{Top-1 accuracy (\%) of various ResNet variants on fine-grained datasets (CUB-200, FGVC-Aircraft, iNat2017/2018) and scenic classification dataset Places205.}
    % \vspace{-4pt}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|cc|cc|c|cc|cc|c|cc}
    \toprule
              & Beta     & \multicolumn{2}{c|}{CUB-200} & \multicolumn{2}{c|}{FGVC-Aircraft} & Beta     & \multicolumn{2}{c|}{iNat2017} & \multicolumn{2}{c|}{iNat2018} & Beta     & \multicolumn{2}{c}{Places205} \\
Method        & $\alpha$ & R-18          & RX-50        & R-18             & RX-50           & $\alpha$ & R-50          & RX-101        & R-50          & RX-101        & $\alpha$ & R-18          & R-50         \\ \hline
Vanilla       & -        & 77.68         & 83.01        & 80.23            & 85.10           & -        & 60.23         & 63.70         & 62.53         & 66.94         & -        & 59.63         & 63.10        \\
MixUp         & 0.2      & 78.39         & 84.58        & 79.52            & 85.18           & 0.2      & 61.22         & 66.27         & 62.69         & 67.56         & 0.2      & 59.33         & 63.01        \\
CutMix        & 1        & 78.40         & 85.68        & 78.84            & 84.55           & 1        & 62.34         & 67.59         & 63.91         & 69.75         & 0.2      & 59.21         & 63.75        \\
ManifoldMix   & 0.5      & 79.76         & 86.38        & 80.68            & 86.60           & 0.2      & 61.47         & 66.08         & 63.46         & 69.30         & 0.2      & 59.46         & 63.23        \\
SaliencyMix   & 0.2      & 77.95         & 83.29        & 80.02            & 84.31           & 1        & 62.51         & 67.20         & 64.27         & 70.01         & 0.2      & 59.50         & 63.33        \\
FMix$^*$      & 0.2      & 77.28         & 84.06        & 79.36            & 86.23           & 1        & 61.90         & 66.64         & 63.71         & 69.46         & 0.2      & 59.51         & 63.63        \\
PuzzleMix     & 1        & 78.63         & 84.51        & 80.76            & 86.23           & 1        & 62.66         & 67.72         & 64.36         & 70.12         & 1        & 59.62         & 63.91        \\
ResizeMix$^*$ & 1        & 78.50         & 84.77        & 78.10            & 84.0            & 1        & 62.29         & 66.82         & 64.12         & 69.30         & 1        & 59.66         & 63.88        \\
AutoMix       & 2        & 79.87         & 86.56        & 81.37            & 86.72           & 2        & 63.08         & 68.03         & 64.73         & 70.49         & 2        & 59.74         & 64.06        \\
SAMix$^*$     & 2        & 81.11         & 86.83        & 82.15            & 86.80           & 2        & 63.32         & 68.26         & 64.84         & 70.54         & 2        & 59.86         & 64.27        \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:app_fgvc_place}
\end{table}

==> tables/app_datasets.tex <==
\begin{table}[b!]
    \centering
    \vspace{-1.25em}
    \caption{Details of benchmarking datasets.}
    % \vspace{-4pt}
\resizebox{0.90\linewidth}{!}{
    \begin{tabular}{l|ccccc}
    \toprule
    Datasets        & Category                 & Classes & Resolution     & Train images & Test images \\ \hline
    ImageNet-1k     & Iconic                   & 1000    & 469$\times$387 & 1,281,167    & 50,000      \\
    CIFAR-10        & Iconic                   & 10      & 32$\times$32   & 50,000       & 10,000      \\
    CIFAR-100       & Iconic                   & 100     & 32$\times$32   & 50,000       & 10,000      \\
    Tiny-ImageNet   & Iconic                   & 200     & 64$\times$64   & 10,000       & 10,000      \\
    CUB-200         & Fine-grained             & 200     & 224$\times$224 & 5,994        & 5,794       \\
    FGVC-Aircraft   & Fine-grained             & 100     & 224$\times$224 & 6,667        & 3,333       \\
    iNaturalist2017 & Fine-grained \& longtail & 5089    & 224$\times$224 & 579,184      & 95,986      \\
    iNaturalist2018 & Fine-grained \& longtail & 8142    & 224$\times$224 & 437,512      & 24,426      \\
    Places205       & Scenic                   & 205     & 224$\times$224 & 2,448,873    & 41,000      \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:app_datasets}
\end{table}

==> tables/tab_fgcls.tex <==
\begin{table}[H]
    \caption{Top-1 accuracy (\%) on IN-1k using PyTorch-style, RSB A2/A3, and DeiT training settings based on CNN and Transformer architectures, including ResNet (R), MobileNet.V2 (Mob.V2), DeiT, and Swin.}
    % \vspace{-4pt}
    \setlength{\tabcolsep}{1.3mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Backbones     & R-50    & R-50   & Mob.V2 1x & DeiT-S & Swin-T \\ \hline
    Epochs        & 100 ep  & 100 ep & 300 ep    & 300 ep & 300 ep \\
    Settings      & PyTorch & RSB A3 & RSB A2    & DeiT   & DeiT   \\ \hline
    Vanilla       & 76.83   & 77.27  & 71.05     & 75.66  & 80.21  \\
    MixUp         & 77.12   & 77.66  & 72.78     & 77.72  & 81.01  \\
    CutMix        & 77.17   & 77.62  & 72.23     & 80.13  & 81.23  \\
    DeiT / RSB    & 77.35   & 78.08  & 72.87     & 79.80  & 81.20  \\
    ManifoldMix   & 77.01   & 77.78  & 72.34     & 78.03  & 81.15  \\
    AttentiveMix+ & 77.28   & 77.46  & 70.30     & 80.32  & 81.29  \\
    SaliencyMix   & 77.14   & 77.93  & 72.07     & 79.88  & 81.37  \\
    FMix*         & 77.19   & 77.76  & 72.79     & 80.45  & 81.47  \\
    PuzzleMix     & 77.54   & 78.02  & 72.85     & 77.37  & 79.60  \\
    ResizeMix*    & 77.42   & 77.85  & 72.50     & 78.61  & 81.36  \\
    AutoMix       & 77.91   & 78.44  & 73.19     & 80.78  & 81.80  \\
    SAMix*        & 78.06   & 78.64  & 73.42     & 80.94  & 81.87  \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:cls_in1k}
\end{table}

